FLINT: A Platform for Federated Learning Integration

Cross-device federated learning (FL) has been well-studied from algorithmic, system scalability, and training speed perspectives. Nonetheless, moving from centralized training to cross-device FL for millions or billions of devices presents many risks, including performance loss, developer inertia, poor user experience, and unexpected application failures. In addition, the corresponding infrastructure, development costs, and return on investment are difficult to estimate. In this paper, we present a device-cloud collaborative FL platform that integrates with an existing machine learning platform, providing tools to measure real-world constraints, assess infrastructure capabilities, evaluate model training performance, and estimate system resource requirements to responsibly bring FL into production. We also present a decision workflow that leverages the FL-integrated platform to comprehensively evaluate the trade-offs of cross-device FL and share our empirical evaluations of business-critical machine learning applications that impact hundreds of millions of users.

==> references.tex <==
MLSYS Program committee: https://mlsys.org/Conferences/2023/ProgramCommittee


On Large-Cohort Training for Federated Learning
https://arxiv.org/pdf/2106.07820.pdf

FEDERATED LEARNING FOR MOBILE KEYBOARD PREDICTION
https://arxiv.org/pdf/1811.03604.pdf


LEARNING COMPRESSED EMBEDDINGS FOR ON-DEVICE INFERENCE
https://arxiv.org/pdf/2203.10135.pdf

Back to the Drawing Board:
A Critical Evaluation of Poisoning Attacks on
Production Federated Learning 
https://arxiv.org/pdf/2108.10241.pdf

Mozilla paper:
https://arxiv.org/pdf/1911.11807.pdf

LinkedIn paper:
https://arxiv.org/pdf/2108.08252.pdf


https://engineering.linkedin.com/blog/2022/challenges-and-practical-lessons-from-building-a-deep-learning-b
